BlinkVision: A Benchmark for Optical Flow, Scene Flow and Point Tracking Estimation using RGB Frames and Events

Recent advances in event-based vision suggest that these systems complement traditional cameras by providing continuous observation without frame rate limitations and a high dynamic range, making them well-suited for correspondence tasks such as optical flow and point tracking. However, there is still a lack of comprehensive benchmarks for correspondence tasks that include both event data and images. To address this gap, we propose BlinkVision, a large-scale and diverse benchmark with multiple modalities and dense correspondence annotations. BlinkVision offers several valuable features: 1) Rich modalities: It includes both event data and RGB images. 2) Extensive annotations: It provides dense per-pixel annotations covering optical flow, scene flow, and point tracking. 3) Large vocabulary: It contains 410 everyday categories, sharing common classes with popular 2D and 3D datasets like LVIS and ShapeNet. 4) Naturalistic: It delivers photorealistic data and covers various naturalistic factors, such as camera shake and deformation. BlinkVision enables extensive benchmarks on three types of correspondence tasks (optical flow, point tracking, and scene flow estimation) for both image-based and event-based methods, offering new observations, practices, and insights for future research. The benchmark website is https://www.blinkvision.net/.

==> tables/category_detail.tex <==



\begin{table}[tb]
\caption{\textbf{Performance evaluation for typical categories at each difficult level.}}
% \vspace{-0.5em}
\centering
\scriptsize
% \footnotesize
\setlength\tabcolsep{2.5pt}
\begin{tabular}{l||cc||cc||cc}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{2}{c}{Hard} & \multicolumn{2}{c}{Medium} & \multicolumn{2}{c}{Easy} \\ 
\cline{2-3} \cline{4-5} \cline{6-7} 
 & person & tree & bench & lantern & notebook & painting \\ \bottomrule
RAFT~\cite{raft} & 9.82 & 9.79 & 4.29 & 2.44 & 1.08 & 0.31 \\
FlowFormer~\cite{flowformer} & 8.72 & \textbf{9.76} & \textbf{3.60} & \textbf{1.92} & \textbf{0.57} & 0.30 \\
FlowFormer++~\cite{shi2023flowformer++} & \textbf{8.61} & 10.10 & 3.68 & 1.95 & 0.84 & \textbf{0.26} \\ \midrule
\end{tabular}
% \vspace{-1.5em}
\label{tab:semantic}
\end{table}

==> tables/event_flow.tex <==
\begin{table}[tb]
\caption{\textbf{Optical flow result of event-based methods.}}
\vspace{-0.5em}
\centering
% \tiny
\footnotesize
\setlength\tabcolsep{3.2pt}
\begin{tabular}{l||ccccc}
\toprule
\multicolumn{6}{c}{Event} \\ \midrule
Methods & Stride-1 & Stride-2 & Stride-4 & Stride-8 & Avg. \\ \midrule
E-RAFT~\cite{eraft} & 2.81 & 7.04 & 17.82 & \textbf{28.60} & 14.07 \\
STE-FlowNet~\cite{ste_flownet} & 2.59 & 5.94 & 13.13 & 41.89 & 15.89 \\
E-FlowFormer~\cite{blinkflow} & \textbf{2.41} & \textbf{5.66} & \textbf{12.53} & 30.45 & \textbf{12.76} \\ \midrule
E-RAFT\dag~\cite{eraft} & 1.68 & 3.63 & 7.48 & 14.20 & 6.75 \\
E-FlowFormer\dag~\cite{blinkflow} & \textbf{1.51} & \textbf{3.00} & \textbf{5.96} & \textbf{13.60} & \textbf{6.02} \\ \midrule
\multicolumn{6}{c}{Event + RGB (clean)} \\ \midrule
Methods & Stride-1 & Stride-2 & Stride-4 & Stride-8 & Avg. \\ \midrule
DCEIFlow~\cite{dceiflow} & 3.31 & 14.07 & 34.78 & 61.56 & 28.43 \\
DCEIFlow\dag~\cite{dceiflow} & \textbf{2.19} & \textbf{6.30} & \textbf{12.54} & \textbf{26.11} & \textbf{11.79} \\ \midrule
\multicolumn{6}{c}{Event + RGB (final)} \\ \midrule
Methods & Stride-1 & Stride-2 & Stride-4 & Stride-8 & Avg. \\ \midrule
DCEIFlow~\cite{dceiflow} & 4.08 & 14.24 & 34.54 & 61.27 & 28.53 \\
DCEIFlow\dag~\cite{dceiflow} & \textbf{2.52} & \textbf{6.86} & \textbf{13.64} & \textbf{28.45} & \textbf{12.87} \\ \bottomrule
\end{tabular}
% \vspace{-1.5em}
\label{tab:event_flow}
\end{table}

==> tables/event_particle.tex <==
\begin{table}[tb]
\caption{\textbf{Point tracking result of event-based methods.} ``*'' denotes that the input is ORB~\cite{orb} feature points.}
\vspace{-0.5em}
\centering
\footnotesize
\setlength\tabcolsep{7pt}
\begin{tabular}{l||ccc}
\toprule
\multicolumn{4}{c}{Event} \\ \midrule
Method & $\delta_\text{avg}$ $\uparrow$ & Survival$\uparrow$ & MTE$\downarrow$ \\ \midrule
AMH~\cite{amh} & 18.95 & 37.98 & 75.44 \\
HASTE~\cite{haste} & 18.60 & 37.43 & 77.36 \\
AMH*~\cite{amh} & 26.76 & 41.93 & 62.48 \\
HASTE*~\cite{haste} & 27.65 & 42.87 & 62.52 \\ \midrule
\multicolumn{4}{c}{Event + RGB (clean)} \\ \midrule
Method & $\delta_\text{avg}$ $\uparrow$ & Survival$\uparrow$ & MTE$\downarrow$ \\ \midrule
Deep-ETracker~\cite{deep_ev_tracker} & 21.62 & 35.44 & 80.80 \\
Deep-ETracker*~\cite{deep_ev_tracker} & \textbf{33.46} & \textbf{48.82} & 60.69 \\ \midrule
\multicolumn{4}{c}{Event + RGB (final)} \\ \midrule
Method & $\delta_\text{avg}$ $\uparrow$ & Survival$\uparrow$ & MTE$\downarrow$ \\ \midrule
Deep-ETracker~\cite{deep_ev_tracker} & 19.05 & 33.52 & 85.00 \\
Deep-ETracker*~\cite{deep_ev_tracker} & 31.78 & 48.67 & \textbf{58.79} \\ \bottomrule
\end{tabular}
% \vspace{-2.0em}
\label{tab:event_particle}
\end{table}

 	 	 	 
 	 	  	 
 	 	 

==> tables/event_scene_flow.tex <==
\begin{table}[bt]
\caption{\textbf{Scene flow result of event-based methods.}}
\vspace{-0.5em}
\centering
\footnotesize
\setlength\tabcolsep{3.2pt}
\begin{tabular}{l|c||cccc}
\toprule
\multicolumn{6}{c}{EPE-2d} \\ \midrule
Method & RGB & Stride-1 & Stride-2 & Stride-4 & Stride-8 \\ \midrule
\multirow{2}{*}{RPEFlow~\cite{rpeflow}} & clean & 1.53 & 3.50 & 7.36 & 17.44 \\
 & final & 1.92 & 4.10 & 8.15 & 18.38 \\ \midrule
\multicolumn{6}{c}{EPE-3d} \\ \midrule
Method & RGB & Stride-1 & Stride-2 & Stride-4 & Stride-8 \\ \midrule
\multirow{2}{*}{RPEFlow~\cite{rpeflow}} & clean & 5.08 & 9.07 & 15.77 & 25.24 \\
 & final & 5.20 & 9.38 & 15.67 & 25.03 \\ \bottomrule
\end{tabular}
% \vspace{-1.5em}
\label{tab:event_scene_flow}
\end{table}

==> tables/finetune.tex <==


\begin{table}[bt]
\caption{\textbf{Cross-dataset evaluation of optical flow methods fine-tuned on BlinkVision.} ``BV'' denotes BlinkVision.}
\vspace{-0.5em}
\centering
\scriptsize
% \footnotesize
\setlength\tabcolsep{3.2pt}
\begin{tabular}{l|c||ccc}
\toprule
\multicolumn{5}{c}{RGB} \\ \midrule
Method & Data & Sintel (clean) & Sintel (final) & KITTI \\ \midrule
\multirow{2}{*}{RAFT~\cite{raft}} & - & 2.08 & 3.41 & 5.10 \\
 & +BV & \textbf{1.69} & \textbf{3.04} & \textbf{4.66} \\ \midrule
\multicolumn{5}{c}{Events} \\ \midrule
Method & Data & E-Blender & FlyingObjects & E-Tartan \\ \midrule
\multirow{2}{*}{E-RAFT~\cite{eraft}} & - & 2.66 & 2.9 & 3.27 \\
 & +BV & \textbf{1.92} & \textbf{2.67} & \textbf{2.55} \\ \midrule
\multirow{2}{*}{E-FlowFormer~\cite{blinkflow}} & - & 2.38 & 2.89 & 2.91 \\
 & +BV & \textbf{1.75} & \textbf{2.58} & \textbf{2.36} \\ \midrule
\multicolumn{5}{c}{Events + RGB} \\ \midrule
Method & Data & E-Blender & FlyingObjects & E-Tartan \\ \midrule
\multirow{2}{*}{DCEIFlow~\cite{dceiflow}} & - & 8.96 & 9.58 & 7.44 \\
 & +BV & \textbf{4.76} & \textbf{2.37} & \textbf{2.88} \\ \bottomrule
\end{tabular}
\label{tab:finetune}
% \vspace{-2.0em}
\end{table}

==> tables/rgb_flow.tex <==
\begin{table}[tb]
\caption{\textbf{Optical flow result of RGB-frame-based methods.} '\dag' denotes the model is finetuned on our train set.}
\vspace{-0.5em}
\centering
% \tiny
\footnotesize
\setlength\tabcolsep{3.2pt}
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{5}{c}{EPE - clean} \\ \cline{2-6} 
 & Stride-1 & Stride-2 & Stride-4 & Stride-8 & Avg. \\ \midrule
RAFT~\cite{raft} & 1.83 & 4.62 & 10.18 & 20.46 & 9.27 \\
GMA~\cite{gma} & 1.82 & 4.37 & 9.52 & 18.68 & 8.60 \\
FlowFormer~\cite{flowformer} & 1.60 & 3.77 & 7.57 & 16.03 & 7.24 \\
FlowFormer++~\cite{shi2023flowformer++} & \textbf{1.54} & \textbf{3.57} & \textbf{7.43} & \textbf{16.26} & \textbf{7.20} \\ \midrule
RAFT\dag~\cite{raft} & 1.33 & 2.96 & 6.39 & 12.72 & 5.85 \\
FlowFormer++\dag~\cite{shi2023flowformer++} & \textbf{1.09} & \textbf{2.35} & \textbf{4.88} & \textbf{10.58} & \textbf{4.73} \\ \midrule
\multirow{2}{*}{Method} & \multicolumn{5}{c}{EPE - final} \\ \cline{2-6} 
 & Stride-1 & Stride-2 & Stride-4 & Stride-8 & Avg. \\ \midrule
RAFT~\cite{raft} & 2.54 & 5.69 & 11.27 & 22.67 & 10.54 \\
GMA~\cite{gma} & 2.56 & 5.72 & 11.21 & 21.35 & 10.21 \\
FlowFormer~\cite{flowformer} & 2.26 & 4.80 & 9.24 & 18.23 & 8.63 \\
FlowFormer++~\cite{shi2023flowformer++} & \textbf{2.28} & \textbf{4.83} & \textbf{9.39} & \textbf{19.08} & \textbf{8.90} \\ \midrule
RAFT\dag~\cite{raft} & 1.94 & 3.88 & 7.35 & 15.17 & 7.08 \\
FlowFormer++\dag~\cite{shi2023flowformer++} & \textbf{1.66} & \textbf{3.34} & \textbf{6.42} & \textbf{12.73} & \textbf{6.04} \\ \bottomrule
\end{tabular}
% \vspace{-1.5em}
\label{tab:rgb_flow}
\end{table}

==> tables/rgb_flow_occ.tex <==

\begin{table}[bt]
\caption{\textbf{Optical flow results of FlowFormer++~\cite{shi2023flowformer++} in different regions.} ``Noc'', ``Occ-in'' and ``Occ-out'' denotes non-occluded regions, in-frame occlusion regions and  out-of-frame occlusion regions, respectively.}
\vspace{-0.5em}
\centering
\scriptsize
% \setlength\tabcolsep{3.2pt}
\begin{tabular}{lccccc}
\toprule
Type & Stride-1 & Stride-2 & Stride-4 & Stride-8 & Avg. \\ \midrule
Noc & 0.96 & 1.89 & 3.70 & 9.41 & 3.99 \\
Occ-in & 3.11 & 5.42 & 9.53 & 17.50 & 8.89 \\
Occ-out & 3.74 & 8.57 & 16.92 & 31.50 & 15.18 \\ \bottomrule
\end{tabular}
% \vspace{-2.0em}
\label{tab:rgb_flow_occ}
\end{table}

==> tables/rgb_particle_rgb_type.tex <==
\begin{table}[tb]
\caption{\textbf{Point tracking result of RGB-frame-based methods under different types of RGB.}}
\centering
% \setlength\tabcolsep{3.2pt}
\footnotesize
\begin{tabular}{l|c||ccc}
\toprule
Method & RGB Type & $\delta_\text{avg}$ $\uparrow$ & Survival$\uparrow$ & MTE$\downarrow$ \\ \midrule
\multirow{2}{*}{PIPs~\cite{pips}} & clean & 37.77 & 52.28 & 50.77 \\
 & final & 33.02 & 48.35 & 53.94 \\ \midrule
\multirow{2}{*}{PIPs++~\cite{pointodyssey}} & clean & \textbf{40.02} & \textbf{53.44} & \textbf{45.51} \\
 & final & \textbf{35.83} & \textbf{50.47} & \textbf{48.37} \\ \midrule
\multirow{2}{*}{Context-TAP~\cite{bian2023context}} & clean & 38.75 & 49.98 & 51.46 \\
 & final & 33.46 & 45.58 & 55.09 \\ \bottomrule
\end{tabular}
\label{tab:rgb_particle_rgb_type}
\end{table}

==> tables/rgb_particle_stride.tex <==
\begin{table}[tb]
\caption{\textbf{Point tracking result of RGB-frame-based methods under different frame interval.}}
\centering
\setlength\tabcolsep{3.2pt}
\footnotesize
\begin{tabular}{l|c||ccccc}
\toprule
Method & Metric & Stride-1 & Stride-2 & Stride-4 & Stride-8 & Avg. \\ \midrule
\multirow{3}{*}{PIPs~\cite{pips}} & $\delta_\text{avg}$ & 37.77 & 39.34 & 36.34 & 25.50 & 34.74 \\
 & Survival$\uparrow$ & 52.28 & \textbf{55.39} & \textbf{54.55} & \textbf{47.58} & \textbf{52.45} \\
 & MTE$\downarrow$ & 50.77 & \textbf{47.81} & \textbf{49.53} & \textbf{62.42} & \textbf{52.63} \\ \midrule
\multirow{3}{*}{PIPs++~\cite{pointodyssey}} & $\delta_\text{avg}$ & \textbf{40.02} & 38.25 & 30.24 & 16.84 & 31.34 \\
 & Survival$\uparrow$ & \textbf{53.44} & 53.13 & 47.57 & 39.71 & 48.46 \\
 & MTE$\downarrow$ & \textbf{45.51} & 51.02 & 59.87 & 73.17 & 57.39 \\ \midrule
\multirow{3}{*}{\makecell{Context-TAP\\~\cite{bian2023context}}} & $\delta_\text{avg}$ & 38.75 & \textbf{39.47} & \textbf{36.51} & \textbf{25.99} & \textbf{35.18} \\
 & Survival$\uparrow$ & 49.98 & 53.09 & 52.61 & 46.18 & 50.46 \\
 & MTE$\downarrow$ & 51.46 & 49.61 & 51.83 & 64.39 & 54.32 \\ \bottomrule
\end{tabular}
% \vspace{-1.5em}
\label{tab:rgb_particle_stride}
\end{table}

==> tables/rgb_scene_flow.tex <==
\begin{table}[tb]
\caption{\textbf{Scene flow result of RGB-frame-based methods.} In the metric of EPE-3d we use decimeters as the unit.}
\vspace{-0.5em}
\centering
\footnotesize
\setlength\tabcolsep{3.2pt}
\begin{tabular}{l|c||cccc}
\toprule
\multicolumn{6}{c}{EPE-2d} \\ \midrule
Method & RGB & Stride-1 & Stride-2 & Stride-4 & Stride-8 \\ \midrule
\multirow{2}{*}{RAFT-3D~\cite{raft3d}} & clean & \textbf{2.15} & \textbf{4.34} & \textbf{8.59} & \textbf{16.08} \\
 & final & \textbf{3.48} & \textbf{7.29} & \textbf{10.74} & \textbf{18.57} \\ \midrule
\multirow{2}{*}{CamLiFlow~\cite{camliflow}} & clean & 2.79 & 6.05 & 12.34 & 23.89 \\
 & final & 4.28 & 8.28 & 16.30 & 30.61 \\ \midrule
\multicolumn{6}{c}{EPE-3d} \\ \midrule
Method & RGB & Stride-1 & Stride-2 & Stride-4 & Stride-8 \\ \midrule
\multirow{2}{*}{RAFT-3D~\cite{raft3d}} & clean & 1.91 & 3.83 & 7.25 & 12.18 \\
 & final & 2.02 & 3.96 & 7.39 & 14.21 \\ \midrule
\multirow{2}{*}{CamLiFlow~\cite{camliflow}} & clean & \textbf{1.45} & \textbf{2.76} & \textbf{5.36} & \textbf{9.12} \\
 & final & \textbf{1.53} & \textbf{2.88} & \textbf{5.60} & \textbf{9.81} \\ \bottomrule
\end{tabular}
% \vspace{-1.5em}
\label{tab:rgb_scene_flow}
\end{table}
